Sharpen the Spec, Cut the Code: A Case for Generative File System with SYSSPEC

File systems are critical OS components that require constant evolution to support new hardware and emerging application needs. However, the traditional paradigm of developing features, fixing bugs, and maintaining the system incurs significant overhead, especially as systems grow in complexity. This paper proposes a new paradigm, generative file systems, which leverages Large Language Models (LLMs) to generate and evolve a file system from prompts, effectively addressing the need for robust evolution. Despite the widespread success of LLMs in code generation, attempts to create a functional file system have thus far been unsuccessful, mainly due to the ambiguity of natural language prompts. This paper introduces SYSSPEC, a framework for developing generative file systems. Its key insight is to replace ambiguous natural language with principles adapted from formal methods. Instead of imprecise prompts, SYSSPEC employs a multi-part specification that accurately describes a file system's functionality, modularity, and concurrency. The specification acts as an unambiguous blueprint, guiding LLMs to generate expected code flexibly. To manage evolution, we develop a DAG-structured patch that operates on the specification itself, enabling new features to be added without violating existing invariants. Moreover, the SYSSPEC toolchain features a set of LLM-based agents with mechanisms to mitigate hallucination during construction and evolution. We demonstrate our approach by generating SPECFS, a concurrent file system. SPECFS demonstrates equivalent level of correctness to that of a manually-coded baseline across hundreds of regression tests. We further confirm its evolvability by seamlessly integrating 10 real-world features from Ext4. Our work shows that a specification-guided approach makes generating and evolving complex systems not only feasible but also highly effective.

==> case-study.tex <==
\section{Case Study}
\label{s:case-study}

\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{0.98\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs-eval/eval-optimizations.pdf}
        \footnotesize
      \end{minipage}
    \caption{\textbf{Features implemented by SpecFS}.
    }
    %\textit{\giptable acts as the control plane of \os, which supports cross-PU localhost direct call and transparent interception.}}
    \label{fig:eval-opts}
  \end{figure*}

\sys implements 10 features based on AtomFS, as illustrated in Figure~\ref{fig:eval-opts}.
The details are as follows.

\myparagraph{Indirect block.}
The indirect block feature (Figure~\ref{fig:eval-opts}-a) expands the maximum file capacity. 
The last block of a file does not store actual file content but instead holds the block addresses of indirect blocks. 
In this way, the number of blocks actually stored by the file exceeds the maximum block number specified by the file system. 
The modification only requires changes to the file operation module (\texttt{lowlevel\_file}).

\myparagraph{Inline data.}
The inline data feature (Figure~\ref{fig:eval-opts}-b) utilizes the remaining space in the inode block to store file content, thereby compressing the actual space occupied by the file.
Similarly, the modification only requires changes to the file operation module (\texttt{lowlevel\_file}).

\myparagraph{Extent.}
The extent feature (Figure~\ref{fig:eval-opts}-c) improves the performance of file operations by reducing the number of disk I/O operations.
Contiguous blocks are represented using the \texttt{extent} data structure and can be read and written contiguously on the disk. 
This approach reduces the size of metadata and disk I/O operations simultaneously.
The modification involves changes to the file operation module (\texttt{lowlevel\_file}) as well as the inode operation module (\texttt{inode\_management}), which calls these file operations. 
Additionally, it requires initializing the extent during initialization (\texttt{inode\_initialization}).

\myparagraph{Extent and pre-allocation.}
The feature (Figure~\ref{fig:eval-opts}-d) is a combination of two optimizations: extent and pre-allocation (pre-alloc).
Pre-allocation allocates additional blocks when a block is initially allocated. 
When a file actually needs a block, it prioritizes obtaining blocks from these pre-allocated and contiguous blocks. 
This enhances the contiguity of a file's blocks on the disk, thereby optimizing disk I/O performance. 
This feature requires the addition of new modules (\texttt{mballoc} and \texttt{contiguous\_malloc}) to implement the pre-allocation logic, 
which is then integrated with \texttt{lowlevel\_file} to implement the logic of obtaining blocks from the pre-allocated blocks for extents.

\myparagraph{Pre-allocation with red-black tree.}
When a file needs to allocate a block, naive pre-allocation involves traversing an array to locate a free block within the pre-allocated block pool. 
The feature depicted in Figure~\ref{fig:eval-opts}-e further accelerates this traversal process by utilizing a red-black tree. 
It adds the \texttt{rbtree} module to implement red-black tree operations and adjusts the corresponding pre-allocation operations to be based on red-black tree operations.

\myparagraph{Checksum.}
The feature (Figure~\ref{fig:eval-opts}-f) generates a checksum for each file based on its metadata and contents, and verifies the checksum during file operations.
The checksum generation and validation logic is implemented in \texttt{checksum} module and called by other modules.

\myparagraph{Encryption and decryption.}
The feature (Figure~\ref{fig:eval-opts}-g) encrypts and decrypts the contents of a file using the XTEA algorithm~\cite{xtea}.
The writing and reading operations of the file requires encryption and decryption respectively.

\myparagraph{Delayed allocation.}
The feature (Figure~\ref{fig:eval-opts}-h) prioritizes read and write operations of files within a global buffer, thereby reducing the number of I/O operations. 
When the buffer reaches its size limit, it is flushed to the disk in a batch.
Since the buffer is shared among all files, 
locking is required before performing read and write operations on the buffer. 
The definition of the buffer, as well as the read/write and locking operations on the buffer, are implemented in the \texttt{delay\_alloc} module.

\myparagraph{Timestamp.}
The feature (Figure~\ref{fig:eval-opts}-i) adds timestamps to the metadata of files to record their creation, modification, and access times. 
The definition, access, and setting of timestamps are implemented in the \texttt{timestamp} module and are called by the other modules.

\myparagraph{Logging.}
The feature (Figure~\ref{fig:eval-opts}-j) ensures data and metadata are initially written to a log, with subsequent flushing to disk upon the completion of a transaction. 
The full implementation of the feature involves two major parts.
First, we enable atomic write operations with ``Logs'', which act like transactions to enhance crash consistency.
The log is protected by read-write locks, allowing multiple readers or a single writer.
The write syscalls of a log are committed to disk when no active file system operations are in progress.
Second, our read and write operations are prioritized on the log to avoid reading out-of-date data from the disk when the log has not been committed.
This is enabled by a one-to-one mapping between log blocks and actual disk blocks. 
During the flush operation, all modifications are written to the disk, and the corresponding log blocks are then erased.
The feature introduces two modules that implement log transactions (\texttt{log\_trans}) and log read/write operations (\texttt{log\_rw}) respectively.
We further adds transaction markers to each system call, and modifies all read and write operations to disk blocks accordingly.

% The implementation of the feature is divided into two components.
% The first component manages the initiation and completion of each transaction. 
% Each system call's write operations are treated atomically to ensure consistency in the event of a crash. 
% To enable concurrent execution of file system operations, it can group the writes of several system calls into a single transaction. 
% The commit to disk occurs when no active file system operations are in progress.
% The second component manages read and write operations to disk blocks. 
% A one-to-one mapping is maintained between log blocks and actual disk blocks. 
% Upon a read or write request, the system first checks the log blocks for the corresponding data. 
% If the data is absent, a new log block is allocated. 
% During the flush operation, all modifications are written to the disk, and the corresponding log blocks are then erased.
% The feature introduces a logging module to implement these components, adds transaction markers to each system call, 
% and modifies all read and write operations to disk blocks accordingly.

==> tab-apis.tex <==
\begin{table*}[t]
\centering
\setlength{\belowcaptionskip}{5pt}
\setlength{\abovecaptionskip}{5pt}
\caption{\textbf{Comparison of Traditional FS Semantics and LLM-FS Semantics.} \textit{Take Linux FS syscalls as an example.}}
\label{t:apis}
\scriptsize
\begin{tabular}{|l|p{1.45cm}|p{5cm}|p{8.3cm}|}
\hline
\textbf{Category} & \textbf{FS API (Fuse)} & \textbf{Traditional FS Semantics} & \textbf{LLM-FS Semantics} \\ \hline \hline
\multirow[m]{6}{*}{File OPs} 
& open & Opens or creates a file and returns a file descriptor (FD) for subsequent read and write operations. & Opens a file and initiates a session for interaction with LLMs. \\ \cline{2-4} 
& read & Reads data from a file with a FD into a buffer. & Receives responses or processed data from the backend LLM. \\ \cline{2-4} 
& write & Writes data from a buffer to a file with a FD. & Submits data to the backend model for processing, e.g., the written data could be a question or command, and the model returns an answer or execution result. \\ \cline{2-4} 
& (e)poll/select & Wait for the file to be readable or writable. & Wait for the LLM's response (\textit{EPOLLIN}) or wait for the LLM session is ready to submit a new request (\textit{EPOLLOUT}). \\ \cline{2-4} 
& (f)truncate & Truncates a file to a specified length. & Can be used to reduce the size of session data, such as removing specific interactions. \\ \cline{2-4} 
& lseek & Sets the read/write position in a file with a FD. & Used to locate specific results or data segments within a session. \\ \cline{2-4} 
& close & Closes a FD and releases associated resources. & Ends a session, releasing resources and potentially saving state for future use. \\ \hline
\multirow[c]{6}{*}{Structure OPs} 
& rename(at) & Renames a file or directory. & Renames a session file to reflect changes in content or purpose. \\ \cline{2-4} 
& link(at) & Creates a new link (hard link) to an existing file. & Creates a new link to an existing session file (hard link). \\ \cline{2-4} 
& symlink(at) & Creates a new symbolic link to an existing file. & Creates a new symbolic link to an existing session file. \\ \cline{2-4}
& readlink(at) & Reads the contents of a symbolic link. & Reads the contents of a symbolic link. \\ \cline{2-4} 
& mkdir(at) & Creates a new directory. & Creates a new directory. \\ \cline{2-4} 
& unlink(at) & Deletes a file or symbolic link from the filesystem. & Deletes a session file or symbolic link from the filesystem. \\ \hline
\multirow[c]{4}{*}{Perm. \& Stats} 
& chmod & Changes file or directory permissions. & Modifies session file/directory access permissions to control which users or processes can interact with the model or access specific sessions. \\ \cline{2-4} 
& chown & Changes ownership and group of a file. & Changes session file ownership to control model maintenance and updates. \\ \cline{2-4} 
& (f)access(at) & Checks if the calling process has permission to access a specified file. & Checks if a user has permission to perform specific model operations or access model output. \\ \cline{2-4} 
& (f)stat & Retrieves file status information, such as size, creation time, and last modification time. & Retrieves status information for model interactions, such as model type, version, size, and resource usage. \\ \hline
Control 
& ioctl & Controls device behavior. & Controls the behavior of LLM inference by changing configurations. \\ \cline{2-4}
& send/recv & Share an opened file's fd through domain sockets. & Share an opened LLM session's fd through domain sockets. \\ \hline
\end{tabular}
%\vspace{-10pt}
\end{table*}


==> tab-eval-delayed-alloc.tex <==
\begin{table}[tbp]
    \caption{Numbers of IO operations w/wo. delayed allocation. \TODO{Figurize this table?}}
    \vspace{-1mm}
    \begin{center}
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c | c | c}
    
    \toprule
    
     \textbf{Operations} & \textbf{xv6 compilation} & \textbf{Copy QEMU}  & \textbf{Large file} & \textbf{Small file}\\
    \hline
    
    \textbf{Data reads} & 589/742 & 0/0 & 12484/2560 & 9987/10000 \\
    \hline
       
    \textbf{Data writes} & 14/21830 & 1644/420918  & 10004/30720 & 78/20000 \\
    \bottomrule
    

    \end{tabular}}
    
    \label{tab:eval-delayed-alloc}
    \end{center}
\end{table}

==> tab-eval-extent.tex <==
\begin{table}[tbp]
    \caption{Numbers of IO operations w/wo. extent. \TODO{Figurize this table?}}
    \vspace{-1mm}
    \begin{center}
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c | c | c}
    
    \toprule
    
     \textbf{Operations} & \textbf{xv6 compilation} & \textbf{Copy QEMU}  & \textbf{Large file} & \textbf{Small file}\\
    \hline
    
    \textbf{Metadata reads} & 23162/32579 & 153578/230367 & 43520/43520 & 30000/40000 \\
    \hline 
    
    \textbf{Metadata writes} & 1583/1519 & 76789/76789 & 2560/2560 & 10000/10000 \\
    \hline
    
    \textbf{Data reads} & 715/742 & 0/0 & 2560/2560 & 10000/10000 \\
    \hline
    
    \textbf{Data writes} & 11362/21830 &  210459/420918 & 20480/30720 & 10000/10000 \\
    \bottomrule
    

    \end{tabular}}
    
    \label{tab:eval-extent}
    \end{center}
\end{table}

==> tab-eval-inline.tex <==
\begin{table}[tbp]
    \caption{File sizes (number of pages) w/wo. inline data.}
    \vspace{-1mm}
    \begin{center}
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c}
    
    \toprule
    
    \textbf{Files}  & \textbf{With Inline Data} & \textbf{Without Inline Data}  \\
    \hline
    
    \textbf{QEMU-10.0.0}~\cite{qemu} & 135870 & 210459 \\
    \hline
    
    \textbf{Linux-6.14.4}~\cite{linux-src}  & 328186 & 415175 \\
    \bottomrule
    

    \end{tabular}}
    
    \label{tab:eval-inline-data}
    \end{center}
\end{table}

==> tab-eval-rbtree.tex <==
\begin{table}[tbp]
    \caption{Access times to the pre-allocation pool.}
    \vspace{-1mm}
    \begin{center}
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c}
    
    \toprule
    
    \textbf{Workloads}  & \textbf{Red-black tree} & \textbf{Linked list}  \\
    \hline
    
    \textbf{5M file, 500 random writes} & 3122 & 6079 \\
    \hline
    
    \textbf{20M file, 1000 random writes}  & 9279 & 48199 \\
    \bottomrule
    

    \end{tabular}}
    
    \label{tab:eval-rbtree}
    \end{center}
\end{table}

==> tab-motiv-patch-type.tex <==
\begin{table}[tbp]
    \caption{Patch Type Classification.}
    \label{tab:motiv-patch-type}
    \centering
    \small
    \renewcommand\arraystretch{1.1}
    \begin{tabularx}{0.95\linewidth}{l | >{\raggedright\arraybackslash}X}
        \toprule
        \textbf{Patch Type} & \textbf{Description} \\
        \midrule
        \textbf{Bug} & Fixes an existing bug \\
        \midrule
        \textbf{Performance} & Proposes a more efficient design or implementation \\
        \midrule
        \textbf{Reliability} & Improves file system robustness \\
        \midrule
        \textbf{Feature} & Implements a new feature \\
        \midrule
        \textbf{Maintenance} & Refactors code, improves documentation without changing semantic behavior \\
        \bottomrule
    \end{tabularx}
\end{table}
